Gaussian Eigen Models for Human Heads

Current personalized neural head avatars face a trade-off: lightweight models lack detail and realism, while high-quality, animatable avatars require significant computational resources, making them unsuitable for commodity devices. To address this gap, we introduce Gaussian Eigen Models (GEM), which provide high-quality, lightweight, and easily controllable head avatars. GEM utilizes 3D Gaussian primitives for representing the appearance combined with Gaussian splatting for rendering. Building on the success of mesh-based 3D morphable face models (3DMM), we define GEM as an ensemble of linear eigenbases for representing the head appearance of a specific subject. In particular, we construct linear bases to represent the position, scale, rotation, and opacity of the 3D Gaussians. This allows us to efficiently generate Gaussian primitives of a specific head shape by a linear combination of the basis vectors, only requiring a low-dimensional parameter vector that contains the respective coefficients. We propose to construct these linear bases (GEM) by distilling high-quality compute-intense CNN-based Gaussian avatar models that can generate expression-dependent appearance changes like wrinkles. These high-quality models are trained on multi-view videos of a subject and are distilled using a series of principal component analyses. Once we have obtained the bases that represent the animatable appearance space of a specific human, we learn a regressor that takes a single RGB image as input and predicts the low-dimensional parameter vector that corresponds to the shown facial expression. In a series of experiments, we compare GEM's self-reenactment and cross-person reenactment results to state-of-the-art 3D avatar methods, demonstrating GEM's higher visual quality and better generalization to new expressions.

==> tables/quantitative_all.tex <==
\begin{table}[]
  \centering
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \caption{Evaluation on novel expressions and views shows on-par results with GA StyleUnet \cite{Li2023AnimatableGL} despite much smaller architecture.}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{l|rrrr}
        Method & PSNR $\uparrow$ & LPIPS $\downarrow$ & SSIM $\uparrow$ & L1 $\downarrow$ \\
        \midrule
        Ours PCA                             & \textbf{32.6781} & \textbf{0.0675} & \textbf{0.9633} & \textbf{0.0069} \\
        Ours Net                             & 29.2454 & 0.0777 & 0.9448 & 0.0096 \\
        GA (CNN) \cite{Li2023AnimatableGL}   & 29.0114 & 0.0812 & 0.9429 & 0.0099 \\
        GA \cite{Qian2023GaussianAvatarsPH}  & 28.3137 & 0.0815 & 0.9433 & 0.0102 \\  
        INSTA \cite{Zielonka2022InstantVH}   & 27.9181 & 0.1153 & 0.9340 & 0.0128 \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:color_errors_test}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \caption{Novel viewpoint evaluation is conducted on a withhold camera from the 16 cameras used for training. Note that the expression has been seen during training, and only the view is new.}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{l|rrrr}
        Method & PSNR $\uparrow$ & LPIPS $\downarrow$ & SSIM $\uparrow$ & L1 $\downarrow$ \\
        \midrule
        Ours PCA                             & \textbf{33.5528} & \textbf{0.0678} & \textbf{0.9662} & \textbf{0.0061} \\
        Ours Net                             & 32.4622 & 0.0713 & 0.9617 & 0.0067 \\
        GA (CNN) \cite{Li2023AnimatableGL}   & 32.4166 & 0.0712 & 0.9614 & 0.0066 \\
        GA \cite{Qian2023GaussianAvatarsPH}  & 31.3197 & 0.0786 & 0.9567 & 0.0075 \\
        INSTA \cite{Zielonka2022InstantVH}   & 27.7786 & 0.1232 & 0.9294 & 0.0163 \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:color_errors_novel}
  \end{minipage}
\end{table}

